A Block Belief-Propagation Algorithm for the Contraction of Tensor-Networks

Simulating many-body quantum systems on a classical computer is difficult due to the large number of degrees of freedom, causing the computational complexity to grow exponentially with system size. Tensor Networks (TN) is a framework that breaks down large tensors into a network of smaller tensors, enabling efficient simulation of certain many-body quantum systems. To calculate expectation values of local observables or simulate nearest-neighbor interactions, a contraction of the entire network is needed. This is a known hard problem, which cannot be done exactly for systems with spatial dimension D>1 and is the major bottleneck in all tensor-network based algorithms. Various approximate-contraction algorithms have been suggested, all with their strengths and weaknesses. Nevertheless, contracting a 2D TN remains a major numerical challenge, limiting the use of TN techniques for many interesting systems. Recently, a close connection between TN and Probabilistic Graphical Models (PGM) has been shown. In the PGM framework, marginals of complicated probability distributions can be approximated using iterative message passing algorithms such as Belief Propagation (BP). The BP algorithm can be adapted to the TN framework as an efficient contraction algorithm. While BP is extremely efficient and easy to parallelize, it often yields inaccurate results for highly correlated quantum states or frustrated systems. To overcome this, we suggest the BlockBP algorithm, which coarse-grains the system into blocks and performs BP between them. This thesis focuses on: (i) development and implementation of the BlockBP algorithm for infinite lattices; (ii) using this algorithm to study the anti-ferromagnetic Heisenberg model on the Kagome lattice in the thermodynamic limit - a frustrated 2D model that is difficult to simulate using existing numerical methods.

==> Chapters/acknowledgments.tex <==
% Define a custom environment with no identation and new line after each paragraph:
\newenvironment{acknowledgementsEnv}{
    \setlength{\parindent}{0pt}
    \setlength{\parskip}{1em}
    \begin{flushleft}
}{
    \end{flushleft}
}


\begin{acknowledgementsEnv}


% \nnote{Remember removing acknowledgements for official first submission}


I would like to express my sincere gratitude to all those who have contributed to the successful completion of my master’s thesis.


First and foremost, I would like to express my deepest appreciation to my supervisors, Professor Anna Keselman and Professor Itai Arad. Their invaluable guidance, support, and expertise throughout this journey had made this achievement possible.  

I am immensely grateful to my beloved wife, Noa, for her unwavering love, support, and patience. She has been my constant source of encouragement, even during the most challenging times. I also wish to acknowledge the newest addition to our family, Tom, who, though not yet a month old, has brought immense joy and love into this thesis journey.

I would like to extend my sincere thanks to Roy Elkabetz and Juraj Hasik for their invaluable insights and assistance with specific questions. I am also deeply grateful to Inbar Kazes and Omer Gurevich, with whom I have shared my office and much of my time while working on this thesis.

To everyone who has supported me in any way, I am truly grateful. Your encouragement and belief in me have made this accomplishment possible.

\end{acknowledgementsEnv}


==> hebrew/habstract.tex <==
עבודה זו מציגה את הפיתוח והיישום של אלגוריתם התפשטות-אמונה על בלוקים 
(Block-Belief-Propagation)
לכיווץ רשתות טנזוריות, תוך התמקדות בחקר מודל הייזנברג האנטיפרומגנטי על סריג קגומה אינסופי. 

האתגר המרכזי בסימולציה של מערכות קוונטיות רב-גופיות על מחשבים קלאסיים נובע מהגידול המעריכי בסיבוכיות החישובית ככל שגודל המערכת גדל. רשתות טנזוריות (TN) מציעות מסגרת מבטיחה לייצוג וסימולציה יעילה של מערכות קוונטיות מסוימות על ידי פירוק טנזורים גדולים לרשת של טנזורים קטנים יותר וניתנים לניהול.
%
כיווץ רשתות טנזוריות הוא תהליך מרכזי במסגרת זו, שבו טנזורים מחוברים זה לזה דרך אינדקסים משותפים, ויוצרים רשת מורכבת. הכיווץ מאפשר מעבר מרשת טנזורית גדולה לרשת קטנה יותר, תוך שמירה על המידע הקוונטי המקורי. זהו שלב חיוני בחישוב ערכי תצפית של מדידים לוקאליים ובסימולציה של אינטראקציות בין שכנים קרובים. עם זאת, הכיווץ של רשתות טנזוריות דו-ממדיות נותר אתגר נומרי מרכזי, המגביל את השימוש בטכניקות אלו במערכות רבות מעניינות.

אלגוריתם התפשטות-אמונה על בלוקים נועד לשפר באופן משמעותי את היעילות והדיוק של כיווץ רשתות טנזוריות. הוא משיג זאת על ידי חלוקת המערכת לבלוקים וביצוע התפשטות-אמונה בין הבלוקים, תוך התמודדות עם אי-דיוקים הנפוצים בשיטות התפשטות-אמונה מסורתיות, במיוחד במערכות קוונטיות המאופיינות בקורלציות גבוהות ותסכול גיאומטרי. האלגוריתם מאפשר האצה משמעותית בזמן העיבוד באמצעות מקבול חישובים, מה שהופך אותו לכלי רב עוצמה לסימולציה של מערכות קוונטיות גדולות.

סריג קגומה, מבנה דו-ממדי המורכב ממשולשים משותפי קודקוד, ידוע בתסכול הגיאומטרי שלו ובמצב היסוד המורכב שלו. במודל הייזנברג האנטיפרומגנטי, הספינים בסריג קגומה שואפים להסתדר הפוך לשכניהם, אך הסידור למשולשים מונע מכל הספינים לספק את הרצון הזה בו זמנית, מה שמוביל למצב יסוד עם תסכול גבוה וללא מגנטיות סטטית. תוצאות נומריות מהמחקר מצביעות על כך שאלגוריתם התפשטות-אמונה על בלוקים מסמלץ ביעילות את סריג קגומה האינסופי, ומשיג בנאמנות גבוהה הערכה למצב היסוד של מודל הייזנברג האנטיפרומגנטי.

המחקר מתאר גם את יישום התהליך של אבולוציית זמן מדומה (ITE) על מצבים של זוגות שזורים מוטלים (PEPS), המאפשרת מציאת מצבי יסוד של המילטוניאנים קוונטיים על ידי קירוב המערכת למצב האנרגיה הנמוך ביותר שלה. התהליך כולל פירוק המילטונים למרכיבים מקומיים ויישום סדרת פעולות על רשת הטנזורים, תוך שימוש באלגוריתם התפשטות-אמונה על בלוקים כדי לייעל את חישוב הסביבה המקומית של הטנזורים.
אחד היתרונות המרכזיים של אלגוריתם התפשטות-אמונה על בלוקים הוא יכולת ההרחבה וההתאמה שלו. האלגוריתם מתאים הן למערכות סופיות והן למערכות אינסופיות, ומציע יישומים פוטנציאליים בגיאומטריות סריג אחרות ובבעיות בכימיה קוונטית. המחקר מציע להשתמש באלגוריתם התפשטות-אמונה על בלוקים במערכות סופיות, שבהן הוא מצטיין בהשוואה לשיטות מתקדמות אחרות.

בנוסף, האלגוריתם מציע גמישות רבה בהתאמה לגיאומטריות סריג שונות, מה שמאפשר לחוקרים לחקור תופעות קוונטיות מורכבות במגוון רחב של מערכות. היכולת של אלגוריתם התפשטות-אמונה על בלוקים ללכוד קורלציות לטווח ארוך ולהתאים את עצמו בקלות למבנים גיאומטריים שונים, פותחת אפשרויות חדשות לחקר מערכות קוונטיות עם מבנים לא סדירים, כמו גם לבעיות בכימיה קוונטית.

לסיכום, אלגוריתם התפשטות-אמונה על בלוקים מייצג התקדמות משמעותית בסימולציה של מערכות קוונטיות רב-גופיות. היכולת שלו לסמלץ ביעילות מערכות קוונטיות גדולות היא קריטית לקידום ההבנה שלנו של תופעות קוונטיות מורכבות. היישום של האלגוריתם על סריג קגומה לא רק מספק תובנות לגבי מערכת זו, אלא גם מציב תקדים להתמודדות עם בעיות מאתגרות דומות בפיזיקה של חומר מעובה. המחקר מדגיש את החשיבות של פיתוח אלגוריתמים ניתנים להרחבה והתאמה שיכולים להתמודד עם המורכבויות של מערכות קוונטיות, ובכך לסלול את הדרך לפריצות דרך עתידיות בתחום.

באופן כללי, עבודה זו מדגימה את הפוטנציאל של אלגוריתם התפשטות-אמונה על בלוקים לחולל מהפכה בדרך שבה אנו ניגשים לסימולציה של מערכות קוונטיות. על ידי מתן שיטה חזקה ויעילה לכיווץ רשתות טנזוריות, אלגוריתם זה מציע כלי רב ערך לחוקרים המבקשים לחקור את המורכבויות של מערכות קוונטיות רב-גופיות. התובנות שהושגו ממחקר זה עשויות להנחות מחקרים עתידיים ולהניע חדשנות בתחום הפיזיקה הקוונטית, ובסופו של דבר לתרום להבנה מעמיקה יותר של העולם הקוונטי.


המחקר פותח דלתות לחקירה נוספת של אלגוריתם התפשטות-אמונה על בלוקים בגיאומטריות סריג אחרות והמילטוניאנים נוספים. כמו כן, הפוטנציאל לשילוב עם בעיות בכימיה קוונטית ומבנים פחות סדירים מציג הזדמנויות מרתקות לעבודה עתידית.



==> hebrew/hacknowledgments.tex <==
% Define a custom environment with no identation and new line after each paragraph:
\newenvironment{hebrewAcknowledgementsEnv}{
    \setlength{\parindent}{0pt}
    \setlength{\parskip}{1em}
    \begin{flushright}
}{
    \end{flushright}
}




\begin{hebrewAcknowledgementsEnv}
    
ברצוני להביע את תודתי הכנה לכל מי שתרם להשלמת עבודת המאסטר שלי בהצלחה.

ראשית, אני מבקש להביע את הערכתי העמוקה למנחים שלי, פרופסור אנה קסלמן ופרופסור איתי ארד. ההדרכה, התמיכה והמומחיות שלהם לאורך כל הדרך הפכו את ההישג הזה לאפשרי.

אני אסיר תודה לאשתי האהובה, נעה, על אהבתה, תמיכתה וסבלנותה הבלתי מתפשרות. היא הייתה מקור העידוד המתמיד שלי, אפילו בזמנים המאתגרים ביותר. אני גם מבקש להכיר בתוספת החדשה למשפחתנו, תום, שלמרות שהוא טרם בן חודש, הביא שמחה ואהבה עצומה למסע הזה של כתיבת התזה.

ברצוני להודות מקרב לב לרועי אלקבץ ויוראי הסיק על התובנות והסיוע הבלתי ניתנים להחלפה שלהם בשאלות ספציפיות. אני גם אסיר תודה מאוד לעינבר קזס ועומר גורביץ', איתם חלקתי את המשרד שלי ורוב הזמן לאורך העבודה על התזה הזו.

לכל מי שתמך בי בדרך כלשהי, אני אסיר תודה. העידוד והאמונה שלכם בי הפכו את ההישג הזה לאפשרי.

\end{hebrewAcknowledgementsEnv}

